Towards User-Focused Cross-Domain Testing: Disentangling Accessibility, Usability, and Fairness

Fairness testing is increasingly recognized as fundamental in software engineering, especially in the domain of data-driven systems powered by artificial intelligence. However, its practical integration into software development may pose challenges, given its overlapping boundaries with usability and accessibility testing. In this tertiary study, we explore these complexities using insights from 12 systematic reviews published in the past decade, shedding light on the nuanced interactions among fairness, usability, and accessibility testing and how they intersect within contemporary software development practices.

==> tables/addressing.tex <==
\begin{table}
  \caption{Remote Communication Characteristics}
  \label{tab:address}

\begin{tabularx}{\linewidth}{p{1.8cm} X}
\toprule
Strategies & Evidence Examples \\ \hline 

Direct Communication & ``Certain important tasks got missed while communicating through teams. So we had to take a stand to email certain important things so they can be tracked effectively.'' (R105) \newline ``Misunderstandings about technical details happened in the past. By talking to each other again, we were able to clarify the requirements''. (R14) \newline \\

Proactivity & ``With many people needing to discuss the same issue in a production problem, we created a war room to resolve the problem in parallel.'' (R13) \newline ``At times, delays in receiving responses from the client via chat impacted our delivery cadence. To address this issue, we began sending emails with managers copied in to ensure everyone was aware of the need for faster communication.''(P39) \newline \\

Regular Alignment & ``The test/QA analyst is integrated into the development team, working together. This way, we can catch many issues before finalizing the development.'' (P44) \newline ``Because everybody is remote, hence sometimes responses can be delayed. However, with multiple follow up through e-mails and discussion, that is no longer an issue.'' (P115) \\
\bottomrule
\end{tabularx}

\end{table}


==> tables/challenging.tex <==
\begin{table*}
  \caption{Challenging Testing Tasks}
  \label{tab:challenge}

\begin{tabularx}{\linewidth}{p{1.5cm} p{2cm} p{5cm} X}
\toprule
Dimension & Factor & Definition & Evidence Examples \\ \hline 

Skill & Knowledge Acquisition & Software testing professionals must continuously learn and experiment to stay abreast of technologies, techniques, and tools, ensuring the process remains up to date. & P02: \textit{``[...] always having new things to learn.''} \newline P04: \textit{``You need to study and stop to plan and understand the context.''}  \newline P06: \textit{``[...] definition of testing strategies, which involves concepts, knowledge of technologies, processes, and tools.''} \newline \\

 & Communication & Software testing professionals must interpret various artifacts and effectively communicate issues with both the team and the client. & P08: \textit{``Keep the team informed regarding improvements in the test development process.''} \newline P14: \textit{``[...] have good communication skills.''}  \newline P22: \textit{``[...] report to the customer.''} \newline \\

& Knowledge \newline Dissemination & Software testing professionals must actively share knowledge with their peers and support collaboration across quality activities. & P02: \textit{``Guiding people is a challenge, [...] because people learn in different ways.''} \newline \\ \hline 

Environment & Instability & Uncertainties of requirements, priorities, or decisions can cause significant changes in the testing strategy, particularly when they arise in the advanced stages of the development cycle. & P07: \textit{``Changes that occurred when development was at an advanced stage or already completed.''} \newline P25: \textit{``I’m always working with different software versions, and new problems always happen.''}  \newline P26: \textit{``[...] new challenges are presented to us, new priorities, new types of processes and methodologies, new work tools and new ways to solve problems of the most varied types.''} \newline \\

 & Time & Delays in earlier stages of software development, such as programming, often lead to a significant reduction in the time allocated for testing activities. & P06: \textit{``Deadlines often become a relevant challenge in the quality process, and convincing the customer is not always an easy task.''} \newline P10: \textit{``Deadline problems always keep the challenge.''}  \newline P27: \textit{``[...] do everything within the deadline''} \newline \\

& Resources & The absence or lack of resources, such as documentation artifacts, complicates the process of defining strategies, identifying test scenarios, and creating test cases. & P06: \textit{``understand the business rules and technologies involved, most of the time, with little or no documentation.''} \newline P18: \textit{``[lack] of documentation.''} \newline \\ \hline 

Attitude & Individual \newline Responsibility & Pro-activeness to ensure the process remains operational and efficient in terms of quality. & P05: \textit{``[...] high degree of responsibility and trust given to me by the team.''} \newline P24: \textit{``High cost of development and responsibility for the results.''}  \newline P30: \textit{``They require creativity and technical knowledge for the result to be satisfactory.''} \newline \\

 & Individual \newline Commitment & The importance of software testing professionals collaborating with their team.. & P07: \textit{``This requires a high degree of commitment and agility from the QA team.''} \newline P21: \textit{``New features always require [...] involvement so that the tests are well-designed and executed.''} \newline \\ \hline 

Task & Task \newline Interchangeability & The frequency of professionals switching activities increases the challenge, as changing contexts too often demands high levels of concentration. \newline & P05: \textit{``[...] I usually don’t spend two days in a row doing the same activity.''} \newline \\

 & Task \newline Complexity & The importance of software testing professionals collaborating with their team. & P23: \textit{``These are not tasks with such direct answers or solutions, so it’s not just a matter of searching on Google or StackOverflow, for example.''} \newline P29: \textit{``Complex system features [...].''} \\

\bottomrule
\end{tabularx}

\end{table*}


==> tables/characteristics.tex <==
\begin{table}
  \caption{Characteristics of Challenge}
  \label{tab:charac}

\begin{tabularx}{\linewidth}{p{1.5cm} p{2cm} X}
\toprule
Characteristic & Definition & Evidence Examples \\ \hline 

Novelty & Challenge is characterized by introducing new tasks into the routine, typically requiring creativity to complete. & P2: \textit{``The new or the unknown [. . . ] what comes out of the
monotonous.''} \newline P4: \textit{``something that is different from your context and that requires more time for study and planning.''}  \newline P29: \textit{``It is something new, a way to reach the final goal that requires effort, creativity, and skill.''} \newline \\

Adaptation & Challenge is characterized by requiring transformation and change in professionals' routines. & P5: \textit{``Do something that goes beyond my limits and comfort zone.''} \newline P7: \textit{``[. . . ] it is what requires easy adaptation and quick learning.''}  \newline P13: \textit{``I challenge myself and everything that makes me leave my comfort zone.''} \newline \\

Knowledge \newline Demanding & Challenge is characterized by demanding learning, enabling professionals to improve their capabilities. & P20: \textit{``things that require knowledge that you do not yet have.''} \newline P21: \textit{``Everything that goes beyond my knowledge.''}  \newline P28: \textit{``Activities that I have not yet fully mastered.''} \\

\bottomrule
\end{tabularx}

\end{table}


==> tables/concepts.tex <==
\begin{table}[!htp]\centering
\caption{Usability, Accessibility and Fairness Characteristics}
\vspace{-2.5mm}
\label{tab:concepts}
\scriptsize
\begin{tabularx}{\linewidth}{p{1.2cm} p{4.8cm} X}
\midrule
\textbf{Aspect} & \textbf{Characteristics} & \textbf{Key \newline Elements}\\
\midrule

\textbf{Usability}
& - ``the extent to which a system, product or service
can be used by specified users to achieve specified goals with
effectiveness, efficiency, and satisfaction.'' \newline
%- ``a satisfactory level of experience is reached when actions such as turning on a TV set and increasing its volume level are accomplished efficiently.'' \newline
- ``a multiple properties of a user interface (...): Learnability (easy to be learned), Memorability (easy to be remembered), (...) and Satisfaction (pleasant to be used).'' \newline
% - ``Usability plays an indispensable role in affecting usage intention.'' \newline
 - ``an unintended behavior by the product that is noticed by the user and has an effect on the user experience.'' \newline
 - ``Usable software should not only have an attractive user interface, but it should be easy to understand, learn, operate and also control.'' \newline
 - ``a degree of ease to use software technology and having user friendly interface.'' \newline
 - ``Perceived ease of use refers to the degree to which the user expects that using a particular service would be free of effort.'' \newline
% - ``Usability involves understandability, learnability, operability, and attractiveness.'' \newline
 - ``Usability expresses the facility with which users can use a technological artifact to achieve a particular goal.'' \newline
  - ``The usability of a product is pleasant when its
interactions require less effort by the user.''

& Interface \newline \newline Pleasantness \newline \newline Learnability \newline \newline Understandability \newline \newline Ease of Use \\
\midrule 

\textbf{Accessibility}
& - ``the degree to which data can be accessed (...), particularly by people who need
supporting technology or specific configuration because of some disability.'' \newline
- ``requirement that establishes how software and computers can be made accessible to users with various types of impairments.'' \newline
- ``broad and extensible term associated with people who have disabilities, incompetent skills, or situational-induced impairment.'' \newline
- ``people with special needs should be able to access, navigate, interact, and contribute to the information that is available.'' \newline
- ``several accessibility guidelines have been introduced by the government of several countries and various public and private institutes.'' \newline
- ``the needs that each disability needs when interacting with web applications.''

& Support for \newline  Disabilities \newline \newline Accommodation for \newline Impairment \newline \newline 
Promotion of \newline Universality \newline \\
\midrule 

\textbf{Fairness}
& - ``a property of learning-based systems which aims to ensure that the software does not exhibit biases.'' \newline
- ``a fair software should not result in discriminatory outputs or behaviors for inputs relating to certain groups or individuals.'' \newline
- ``ensure a given system produces the same results or exhibits
similar behaviors for a number of discriminatory inputs.'' \newline
- ``requires that software should produce similar predictive outcomes for similar individuals.'' \newline
- ``requires software to treat different demographic groups in a similar manner.'' \newline
- ``profound ethical implications, resulting
in unacceptable outcomes, particularly by disadvantaging minority groups.'' \newline
- ``more challenging because inputs and outputs from different
demographic groups need to be considered simultaneously.'' \newline
- ``an algorithm should not produce unjust, discriminatory, or disparate consequences.'' \newline
- ``embedding societal values in the design of ADM systems.''
%- ``featured in more than 80\% of guidelines for AI ethics.''

& Decrease of \newline Discrimination \newline \newline Treatment of \newline Minorities \newline \newline Ethical \newline Considerations \newline \newline \\

\bottomrule
\end{tabularx}
\end{table}

==> tables/effects.tex <==
\begin{table}
  \caption{Effects of Challenge on Testing Professionals}
  \label{tab:effects}

\begin{tabularx}{\linewidth}{p{1.5cm} p{2cm} X}
\toprule
Effect & Emotions & Evidence Examples \\ \hline 

Positive & Challenges have the potential to elevate excitement, confidence, curiosity, determination, disposition, and happiness. & P6: \textit{`` the challenges usually motivate me more than demotivate.''} \newline P10: \textit{``Motivated, especially when it is possible to see the evolution and growth in the face of this challenge.''}  \newline P25: \textit{``I feel excited and willing to contribute more and more to
the project.''} \newline \\


Negative & Challenges may induce feelings of anxiety, apprehension, disinterest, stress, and worry. & P09: \textit{``[. . . ] worried about the results not meeting the desired level.''} \newline P13: \textit{``I am VERY afraid of not being able to perform well.''}  \newline P28: \textit{``Stressed and anxious, due to the doubt and uncertainties.''} \\

\bottomrule
\end{tabularx}

\end{table}

